Accelerated Patient-Specific Calibration via Differentiable Hemodynamics Simulations

One of the goals of personalized medicine is to tailor diagnostics to individual patients. Diagnostics are performed in practice by measuring quantities, called biomarkers, that indicate the existence and progress of a disease. In common cardiovascular diseases, such as hypertension, biomarkers that are closely related to the clinical representation of a patient can be predicted using computational models. Personalizing computational models translates to considering patient-specific flow conditions, for example, the compliance of blood vessels that cannot be a priori known and quantities such as the patient geometry that can be measured using imaging. Therefore, a patient is identified by a set of measurable and nonmeasurable parameters needed to well-define a computational model; else, the computational model is not personalized, meaning it is prone to large prediction errors. Therefore, to personalize a computational model, sufficient information needs to be extracted from the data. The current methods by which this is done are either inefficient, due to relying on slow-converging optimization methods, or hard to interpret, due to using `black box` deep-learning algorithms. We propose a personalized diagnostic procedure based on a differentiable 0D-1D Navier-Stokes reduced order model solver and fast parameter inference methods that take advantage of gradients through the solver. By providing a faster method for performing parameter inference and sensitivity analysis through differentiability while maintaining the interpretability of well-understood mathematical models and numerical methods, the best of both worlds is combined. The performance of the proposed solver is validated against a well-established process on different geometries, and different parameter inference processes are successfully performed.

==> old_det_inf.tex <==
\begin{equation*}
    \mathbf{y}_i = \mathbf{u}_i(\hat{\xi}).
\end{equation*}

The objective is to solve
For the deterministic estimation we consider measurements $\{ \mathbf{y} \}_{i=1}^N$ at locations $\{ x_i\}_{i=1}^N$ again following the relation:

\begin{equation*}
    \mathbf{y}_i = \mathbf{u}_i(\hat{\xi_i}),
\end{equation*}
and the objective is solve:
\begin{equation*}
    \xi = \min_{\xi \in \Xi} L(\xi),
\end{equation*}
where
\begin{equation*}
    L(\xi) = \frac{1}{N} \sum_{i,j=1}^{N,M} ( y_{ij} - u_{ij}(\hat{\xi_i}) )^2.
\end{equation*}
where $M$ the number of measurements in a single vessel, through a gradient descent strategy:
\begin{equation*}
    \xi^{k+1} = \xi^{k} - \lambda \nabla_{\xi} L(\xi^k), 
\end{equation*}
where the gradient 
\begin{equation*}
     \nabla_{\xi} L(\xi^k) = \frac{2}{N} \sum_{i,j=1}^{N,M} | y_{ij} - u_{ij}(\hat{\xi_i} | \ \nabla_{\xi} u_{ij}(\hat{\xi_i})
\end{equation*}
is computed by performing automatic differentiation through the solver. For this purpose, we consider the Adam optimizer \cite{kingma2014adam} with the default parameter choices. We consider a first the case where only $R_2$ is inferred from data and a second case where $R_2, C_2$ and $R_3, C_3$ are all inferred from data. The results of such an optimization for the first case can be seen in \ref{fig:optax_1}. As in the previous section the baseline parameter is $R_2=6.8123 \times 10^7$. For the optimization the parameter was initialized as randomly from a unifrom distribution $U(0,2)$

\begin{figure}[h!]
\centering
\includegraphics[width=0.4\columnwidth]{figures/optax_1/10_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_1/20_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_1/50_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_1/100_nt.eps}
\caption{Optimization of the $R_1$ parameter with 10, 20, 50, and 100 iterations from top left to bottom right. The Adam optimization already provides accurate results after 10 iterations. After 50 the smallest loss can be observed and further optimization provides no more improvement.}
\label{fig:optax_1}
\end{figure}

\begin{table}[h!]
    \centering
    \begin{tabular}{cccc}
    \hline
         $\#$ Iterations & Log-Loss & Wall-clock Time $[s]$\\
    \hline
        10 & -9.11018 & 16.49112 \\
    \hline
        20 & -14.42231 & 17.26087 \\
    \hline
        50 & -14.59830 & 19.59227 \\
    \hline
        100 & -14.57091 & 23.45158 \\
    \hline
    \end{tabular}
    \caption{We present comparisons using the relative $L_1$ error for the anatomies and the arteries presented in Figure \ref{fig:val}.}
    \label{tab:errors_comp}
\end{table}

The optimization of a single parameter reaches a high level of accuracy after only a few steps and could be stopped way earlier in practice than was done here while still obtaining good enough results.  Here again, as in the stochastic optimization experiments, all four Windkessel resistance parameters of the network were optimized. The results from this procedure can be seen in \ref{fig:optax_4}.
 
\begin{figure} [h!]
\centering
\includegraphics[width=0.4\columnwidth]{figures/optax_4/10_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_4/20_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_4/50_nt.eps}
\includegraphics[width=0.4\columnwidth]{figures/optax_4/100_nt.eps}
\caption{Optimization of Windkessel parameters with 10, 20, 50, and 100 iterations from top left to bottom right. Opposed to the setup where only a single parameter was optimized, even after 50 iterations there is still a clearly visible difference in between the baseline and the prediction. After 100 iterations however, The optimization process still provides very accurate results.}
\label{fig:optax_4}
\end{figure}

% We need to explain the problem setup better and maybe provide a sketch.
% - First describe the anatomy: A single bifurcation. Maybe a sketch.
% - State problem setup, which parameters you are trying to infer. 

We start by considering measurements $\{ \mathbf{y} \}_{i=1}^N$ at locations $\{ x_i\}_{i=1}^N$, which are related to ground-truth measured quantity, for example the velocity $\mathbf{u}_i = \mathcal{H}(\hat{\xi_i})$, where $\mathcal{H}$ the PDE operator that maps the parameters to the observables, through:

\begin{equation*}
    \mathbf{y}_i = \mathbf{u}_i(\hat{\xi_i}) + \mathbf{\epsilon}, \quad \mathbf{\epsilon} \sim  \mathcal{N}(\mathbf{0}, \sigma^2 \mathbf{I})
\end{equation*}
where $\epsilon$ the measurement error, and $\hat{\xi_i} = \{R_i, C_i\}$ the parameters to be identified. The Bayesian probabilistic framework, considers $\hat{\xi_i}$ as a random variable and computes the posterior distribution:

\begin{equation*}
    p( \hat{\xi_i} | \mathbf{y}) =  \frac{p( \mathbf{y} | \hat{\xi_i}) p (\hat{\xi_i})}{ p(\mathbf{y})},
\end{equation*}
where $p( \mathbf{y} | \theta)$ the likelihood probability, $p(\mathbf{y})$ the evidence, and $p (\hat{\xi_i})$ the prior distribution of the parameters. Assuming a the noise to be a Gaussian distribution, we can write the log-likelihood as:

\begin{equation}
\label{eq:likelihood}
   \log p( \mathbf{y}_i | \theta) = \sum_{i=1}^N \log p_{\epsilon} (\mathbf{y}_i - \mathbf{u}_i(\hat{\xi_i}) ). 
 \end{equation}

The evidence probability is intractable to compute and therefore we compute the un-normalized posterior:

\begin{equation}
    \label{eq:posterior}
     p( \hat{\xi_i} | \mathbf{y}) \propto  p( \mathbf{y} | \hat{\xi_i}) p (\hat{\xi_i}).
\end{equation}


To test the probabilistic pipeline, we infer $\{ R_2 \}$ parameter of the Windkessel models at the outlet of vessel $\# 2$. 


We run the solver for the nominal value $\hat{R}_2=6.8123 \times 10^7$ to generate the target pressure $\mathbf{y}$, see Equation \ref{eq:likelihood}. Once the baseline is computed, we consider $\hat{R}_2 = s_c \bar{R}_2$, where $s_c \in [0,1]$ a scale parameter and $\bar{R}_2 = 10^8$ an order of magnitude parameter. Our goal is to find $s_c$ for each parameter. For this purpose, the No-U-Turn Sampler (NUTS) \cite{hoffman2014no} is employed to perform a Hamiltonian Monte Carlo \cite{duane1987hybrid} sampling with adaptive path lengths, using the \emph{NumPyro} \cite{phan2019composable,bingham2019pyro} environment. 

The optimizer was run with 5 warm-up-steps and 15 sample-steps. The parameter inference pipeline took around two minutes and returned a relative $L_2$ error equal to $3.1 \times 10^{-5}$ between the baseline and the pressure for the inferred pressure. The parameter inference took roughly one hour and returned $7 \times 10^7$ as the mean for the posterior of $\bar{R}_1$ leading to a relative error of about $2.5\%$. 




% \subsection{Black-Box Closure Models} \label{sec:bbcm}

